Hidden regularity in singular optimal control of port-Hamiltonian systems

We study the problem of state transition on a finite time interval with minimal energy supply for linear port-Hamiltonian systems. While the cost functional of minimal energy supply is intrinsic to the port-Hamiltonian structure, the necessary conditions of optimality resulting from Pontryagin's maximum principle may yield singular arcs. The underlying reason is the linear dependence on the control, which makes the problem of determining the optimal control as a function of the state and the adjoint more complicated or even impossible. To resolve this issue, we fully characterize regularity of the (differential-algebraic) optimality system by using the interplay of the cost functional and the dynamics. In case of the optimality DAE being characterized by a regular matrix pencil, we fully determine the control on the singular arc. In case of singular matrix pencils of the optimality system, we propose an approach to compute rank-minimal quadratic perturbations of the objective such that the optimal control problem becomes regular. We illustrate the applicability of our results by a general second-order mechanical system and a discretized boundary-controlled heat equation.

==> ex_shared.tex <==
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage[english]{babel}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{paralist}
\usepackage[paper=a4paper,left=25mm,right=25mm,top=25mm,bottom=25mm]{geometry}
\usepackage{hyperref}
\usepackage{color} 
\usepackage{fancyhdr}
\usepackage{nomencl}
\usepackage{cite}
\usepackage{float}
\usepackage{amsopn}
\usepackage{xcolor}
%===============================================================
% Damit Manuels Schaubild funktioniert:
\usepackage{tikz}%{pgfplots,tikz}
\usetikzlibrary{shapes,arrows,decorations.markings,decorations.text}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{calc}
\tikzstyle{block2} = [rectangle, draw, 
text width=25em, text centered, rounded corners, minimum height=6em]
\tikzstyle{block3} = [rectangle, draw, 
text width=30em, text centered, rounded corners, minimum height=4em]
\tikzstyle{block3b} = [rectangle, draw, 
text width=30em, text centered, rounded corners, minimum height=4em]
\tikzstyle{block4} = [rectangle, draw, text width = 18em, text centered, rounded corners, minimum height = 4em]
\tikzstyle{block5} = [rectangle, draw, text width = 18em, text centered, rounded corners, minimum height = 4em]
\tikzstyle{block7} = [rectangle, draw, 
text width=35em, text centered, rounded corners, minimum height=4em]

\tikzstyle{blocktest} = [rectangle, draw, 
text width=30em, text centered, rounded corners, minimum height=4.3em]

\tikzstyle{arrow} = [draw, -latex']
\tikzstyle{line} = [draw, -latex']
%===============================================================

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

\newcommand{\Q}{S}
\newcommand{\PH}{\Sigma_{n,m}}

\newcommand{\rk}{\mathrm{rk}\,}
\newcommand{\im}{\mathrm{im}\,}
\newcommand{\id}{\mathrm{id}\,}
\newcommand{\Res}{\mathrm{Res}}
\newcommand{\ind}{\mathrm{ind}\,}

\newcommand{\norm}[1]{\left\Vert #1 \right\Vert}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\set}[1]{\left\lbrace #1 \right\rbrace}
\newcommand{\sign}{\text{sign }}

\renewcommand{\exp}[1]{e^{#1}}

\renewcommand{\Re}{\mathrm{Re}\,}
\renewcommand{\Im}{\mathrm{Im}\,}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{example}{Example}

% Sets running headers as well as PDF title and authors
\headers{Hidden regularity in optimal control of pH systems%Hidden regularity in singular optimal control of port-Hamiltonian systems
}{T. Faulwasser, J. Kirchhoff, V. Mehrmann, F. Philipp, M. Schaller, K. Worthmann}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Hidden regularity in singular optimal control of port-Hamiltonian systems%Port-Hamiltonian optimal control from the DAE point of view
\thanks{Preprint submitted to Arxiv on 05/05/23}
\funding{JK thanks Technische Universität Ilmenau and Freistaat Thüringen for their financial support as part of the Thüringer Graduiertenförderung. VM was supported by German Research Foundation through Priority Program SPP 1984 \textit{Hybrid and multimodal energy systems} within the project \textit{Distributed Dynamic Security Control}. FP was funded by the Carl Zeiss Foundation within the project \textit{DeepTurb--Deep Learning in and from Turbulence} and by the free state of Thuringia within the project \textit{THInKI--Th\"uringer Hochschulinitiative für KI im Studium}. KW gratefully acknowledges funding by the German Research Foundation (DFG; grant no.\ 507037103).}}
% Authors: full names plus addresses.
\author{
Timm Faulwasser\thanks{Institute of Energy Systems, Energy
Efficiency and Energy Economics, TU Dortmund University,  Germany (\email{timm.faulwasser@ieee.org})}
\and Jonas Kirchhoff\thanks{Optimization-based Control Group, Institute of Mathematics, Technische Universität Ilmenau, Germany
% (\email{jonas.kirchhoff@tu-ilmenau.de}, \email{friedrich.philipp@tu-ilmenau.de}, \email{manuel.schaller@tu-ilmenau.de}, \email{karl.worthmann@tu-ilmenau.de}).
(\{jonas.kirchhoff, friedrich.philipp, manuel.schaller, karl.worthmann\}@tu-ilmenau.de).
}
\and Volker Mehrmann\thanks{Institute of Mathematics, Technische Universität Berlin, Germany (\email{mehrmann@math.tu-berlin.de}), }
\and Friedrich Philipp\footnotemark[3]
\and Manuel Schaller\footnotemark[3]
\and Karl Worthmann\footnotemark[3]}


%------------------------------------------------------------------------------
%
%     FRITZ' DEFINITIONS
%
%------------------------------------------------------------------------------
% Often used
\newcommand{\paragraf}{\textsection}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\Indicator}{\mathds{1}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\braces}[1]{{\rm (}#1{\rm )}}
\newcommand{\rmref}[1]{{\rm\ref{#1}}}
\newcommand{\Id}{\operatorname{Id}}

% Numbers
\newcommand{\R}{\ensuremath{\mathbb R}}    % Reelle Zahlen
\newcommand{\C}{\ensuremath{\mathbb C}}    % Komplexe Zahlen
\newcommand{\CC}{\ensuremath{\mathbb C}}   % Komplexe Zahlen
%\newcommand{\Q}{\ensuremath{\mathbb Q}}    % Rationale Zahlen
\newcommand{\N}{\ensuremath{\mathbb N}}    % Nat"urliche Zahlen
\newcommand{\Z}{\ensuremath{\mathbb Z}}    % Ganze Zahlen
\newcommand{\K}{\ensuremath{\mathbb K}}    % Irgendein Koerper
\newcommand{\T}{\ensuremath{\mathbb T}}    % Einheitskreis


% Inner product stuff
\newcommand{\gperp}{{[\perp]}}
\newcommand{\iso}{\circ}
\newcommand{\product}{[\cdot\,,\cdot]}
\newcommand{\hproduct}{(\cdot\,,\cdot)}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\aperp}{{\langle\perp\rangle}}
\newcommand{\aproduct}{\langle\cdot\,,\cdot\rangle}
\newcommand{\llb}{\llbracket}               % Nur mit package stmaryrd.sty
\newcommand{\rrb}{\rrbracket}               % Nur mit package stmaryrd.sty
\newcommand{\dproduct}{\llb\cdot,\cdot\rrb} % Nur mit package stmaryrd.sty
\newcommand{\dperp}{{\llb\perp\rrb}}        % Nur mit package stmaryrd.sty


% Letters
\newcommand{\calA}{\mathcal A}         \newcommand{\frakA}{\mathfrak A}
\newcommand{\calB}{\mathcal B}         \newcommand{\frakB}{\mathfrak B}
\newcommand{\calC}{\mathcal C}         \newcommand{\frakC}{\mathfrak C}
\newcommand{\calD}{\mathcal D}         \newcommand{\frakD}{\mathfrak D}
\newcommand{\calE}{\mathcal E}         \newcommand{\frakE}{\mathfrak E}
\newcommand{\calF}{\mathcal F}         \newcommand{\frakF}{\mathfrak F}
\newcommand{\calG}{\mathcal G}         \newcommand{\frakG}{\mathfrak G}
\newcommand{\calH}{\mathcal H}         \newcommand{\frakH}{\mathfrak H}
\newcommand{\calI}{\mathcal I}         \newcommand{\frakI}{\mathfrak I}
\newcommand{\calJ}{\mathcal J}         \newcommand{\frakJ}{\mathfrak J}
\newcommand{\calK}{\mathcal K}         \newcommand{\frakK}{\mathfrak K}
\newcommand{\calL}{\mathcal L}         \newcommand{\frakL}{\mathfrak L}
\newcommand{\calM}{\mathcal M}         \newcommand{\frakM}{\mathfrak M}
\newcommand{\calN}{\mathcal N}         \newcommand{\frakN}{\mathfrak N}
\newcommand{\calO}{\mathcal O}         \newcommand{\frakO}{\mathfrak O}
\newcommand{\calP}{\mathcal P}         \newcommand{\frakP}{\mathfrak P}
\newcommand{\calQ}{\mathcal Q}         \newcommand{\frakQ}{\mathfrak Q}
\newcommand{\calR}{\mathcal R}         \newcommand{\frakR}{\mathfrak R}
\newcommand{\calS}{\mathcal S}         \newcommand{\frakS}{\mathfrak S}
\newcommand{\calT}{\mathcal T}         \newcommand{\frakT}{\mathfrak T}
\newcommand{\calU}{\mathcal U}         \newcommand{\frakU}{\mathfrak U}
\newcommand{\calV}{\mathcal V}         \newcommand{\frakV}{\mathfrak V}
\newcommand{\calW}{\mathcal W}         \newcommand{\frakW}{\mathfrak W}
\newcommand{\calX}{\mathcal X}         \newcommand{\frakX}{\mathfrak X}
\newcommand{\calY}{\mathcal Y}         \newcommand{\frakY}{\mathfrak Y}
\newcommand{\calZ}{\mathcal Z}         \newcommand{\frakZ}{\mathfrak Z}

\newcommand{\scrA}{\mathscr A}  % For scr-font package "mathrsfs" is needed
\newcommand{\scrB}{\mathscr B}
\newcommand{\scrC}{\mathscr C}
\newcommand{\scrD}{\mathscr D}
\newcommand{\scrE}{\mathscr E}
\newcommand{\scrF}{\mathscr F}
\newcommand{\scrG}{\mathscr G}
\newcommand{\scrH}{\mathscr H}
\newcommand{\scrI}{\mathscr I}
\newcommand{\scrJ}{\mathscr J}
\newcommand{\scrK}{\mathscr K}
\newcommand{\scrL}{\mathscr L}
\newcommand{\scrM}{\mathscr M}
\newcommand{\scrN}{\mathscr N}
\newcommand{\scrO}{\mathscr O}
\newcommand{\scrP}{\mathscr P}
\newcommand{\scrQ}{\mathscr Q}
\newcommand{\scrR}{\mathscr R}
\newcommand{\scrS}{\mathscr S}
\newcommand{\scrT}{\mathscr T}
\newcommand{\scrU}{\mathscr U}
\newcommand{\scrV}{\mathscr V}
\newcommand{\scrW}{\mathscr W}
\newcommand{\scrX}{\mathscr X}
\newcommand{\scrY}{\mathscr Y}
\newcommand{\scrZ}{\mathscr Z}

\newcommand{\la}{\lambda}
\newcommand{\veps}{\varepsilon}
\newcommand{\eps}{\varepsilon}
\newcommand{\vphi}{\varphi}


% Matrices and vectors
\newcommand{\bmat}[4]
{
   \begin{bmatrix}
      #1 & #2\\
      #3 & #4
   \end{bmatrix}
}
\newcommand{\bvec}[2]
{
   \begin{bmatrix}
      #1\\
      #2
   \end{bmatrix}
}
\newcommand{\sbvec}[2]{\left[\begin{smallmatrix}#1\\#2\end{smallmatrix}\right]}
\newcommand{\sbmat}[4]{\left[\begin{smallmatrix}#1 & #2\\#3 & #4\end{smallmatrix}\right]}
\newcommand{\bmattt}[9]
{
   \begin{bmatrix}
      #1 & #2 & #3\\
      #4 & #5 & #6\\
      #7 & #8 & #9
   \end{bmatrix}
}
\newcommand{\bveccc}[3]
{
   \begin{bmatrix}#1\\#2\\#3\end{bmatrix}
}

% Not in italic mode
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}
\newcommand{\linspan}{\operatorname{span}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\ran}{\operatorname{ran}}


% Arrows
\newcommand{\lra}{\longrightarrow}
\newcommand{\sra}{\rightarrow}
\newcommand{\Lra}{\Longrightarrow}
\newcommand{\Sra}{\Rightarrow}

\newcommand{\lla}{\longleftarrow}
\newcommand{\sla}{\leftarrow}
\newcommand{\Lla}{\Longleftarrow}
\newcommand{\Sla}{\Leftarrow}

\newcommand{\llra}{\longleftrightarrow}
\newcommand{\slra}{\leftrightarrow}
\newcommand{\Llra}{\Longleftrightarrow}
\newcommand{\Slra}{\Leftrightarrow}

\newcommand{\upto}{\uparrow}
\newcommand{\downto}{\downarrow}

\newcommand{\wto}{\rightharpoonup}
\newcommand{\Ato}{\stackrel{A}{\to}}
\newcommand{\Awto}{\stackrel{A}{\rightharpoonup}}
\newcommand{\restr}{\!\!\upharpoonright\!\!}


% Misc
\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}
\newcommand{\directSum}{\dotplus}
\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}


% Only here
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator*{\argmin}{argmin}
